Measuring gravity with milligram levitated masses

Gravity differs from all other known fundamental forces since it is best described as a curvature of spacetime. For that reason it remains resistant to unifications with quantum theory. Gravitational interaction is fundamentally weak and becomes prominent only at macroscopic scales. This means, we do not know what happens to gravity in the microscopic regime where quantum effects dominate, and whether quantum coherent effects of gravity become apparent. Levitated mechanical systems of mesoscopic size offer a probe of gravity, while still allowing quantum control over their motional state. This regime opens the possibility of table-top testing of quantum superposition and entanglement in gravitating systems. Here we show gravitational coupling between a levitated sub-millimeter scale magnetic particle inside a type-I superconducting trap and kg source masses, placed approximately half a meter away. Our results extend gravity measurements to low gravitational forces of attonewton and underline the importance of levitated mechanical sensors. Specifically, at a frequency of 26.7 Hz, a mass of 0.4 mg and showing Q-factors in excess of 10$^7$, we obtained a force noise of 0.5 $fN\sqrt{Hz}$ . We simultaneously detect the other 5 rotational and translational degrees of freedom.

==> Conclusion/Conclusion.tex <==
\section{Conclusions}\label{sec:conclusions}
We demonstrate the detection of a \SI{30}{aN} gravitational signal at \SI{27}{Hz} and a damping linewidth as low as $\gamma/2\pi = \SI{2.9}{\mu Hz}$, with a \SI{0.43}{mg} test mass, paving the way for future experiments in which both source and test mass are in this regime. This work could be used to derive a more stringent bound on dissipative collapse models. Furthermore it provides a promising platform to test for possible deviations from inverse square force laws and fifth force models~\cite{Blakemore2021, smullin2005}, theories of modified Newtonian dynamics~\cite{milgrom1983, bekenstein2004} and other extensions of the standard model~\cite{carney2021}.

By ensuring that the pick-up loop is placed off-centre with respect to the trap and by breaking the rotational symmetry in \textgamma\ we demonstrate detection of all six mechanical modes, in comparison to earlier work. As we will discuss in future work, this is critical to the stability of the mode under test due to non-linear mixing between the different modes.

With a mode temperature of 3 kelvin compared to an operating temperature of 30 millikelvin, we are currently not yet thermally limited.
It would require another 20 dB of vibration isolation to reach thermal motion.

By using a second particle in a different trap as source mass, or a similar construction, this work paves the way towards easily scaleable measurements of gravitational coupling in the hertz regime and with source masses at Planck mass level, ultimately allowing for testing gravity in a yet unexplored low-mass regime and pushing into the quantum controlled domain. Coupling of the detection SQUIDs in this scheme to an superconducting LC circuit would provide a means of inserting single microwave photons, providing access to the toolbox of quantum state manipulation. This would further extend this work towards truly macroscopic superposition measurements and gravitationally-induced entanglement.



==> Introduction/Introduction.tex <==
Einstein’s theory of general relativity (GR), our widely accepted theory of gravity, has seen different experimental confirmations~\cite{Einstein1916,walsh1979} by observing massive astronomical objects and their dynamics, most recently by the direct observation of gravitational waves from the merger of two black holes~\cite{abbott2016} and the imaging of a black hole by the event horizon telescope~\cite{akiyama2019}, as well as dedicated satellite missions for testing the basic principle of GR --- the equivalence principle~\cite{touboul2017} and frame dragging effects~\cite{everitt2011}. Laboratory experiments have been continuously increasing the sensitivity of gravity phenomena, including general relativistic effects in atom clocks and atom interferometers~\cite{bothwell2022, asenbaum2017}, tests of the equivalence principle~\cite{rosi2017, asenbaum2020}, precision measurements of Newton's constant~\cite{rosi2014, quinn2013} and tests of the validity of Newton's law at micrometre-scale distances~\cite{geraci2008, tan2020}. 

However, gravity has never been tested for small masses and on the level of the Planck mass. Measurements of gravity from classical sources in laboratory table-top settings is contrasted by an increasing interest to study gravitational phenomena originating from quantum states of source masses, for example, in the form of the gravitational field generated by a quantum superposition state~\cite{bronstein2012republication, rickles2011role, bose2017, marletto2017, al2018optomechanical}. The effort ultimately aims at directly probing the interplay between quantum mechanics and general relativity in table-top experiments. Because quantum coherence is easily lost for increasing system size, it is important to isolate gravity as a coupling force for as small objects as possible, which in turn means to measure gravitational forces and interactions extremely precisely. 

At the same time, massive quantum sensors are especially suited for tests in a regime with appreciable gravitational influences, which is favourable in probing physical models of the wave function collapse~\cite{diosi2015, vinante2016,bassi2013}, namely those that feature the system mass explicitly, such as the continuous spontaneous localization (CSL) model~\cite{ghirardi1990} and the Di\'{o}si-Penrose model of gravitationally-induced collapse~\cite{diosi1987,penrose1996,oosterkamp2013}.


An emerging technology for ultra-sensitive sensing is based on levitated mechanical systems. These can be used for the mechanical sensing of very weak forces and to probe quantum physics at increasing scales of mass (and space). In optical levitation schemes, the heating from trapping lasers is the most prominent source of noise. Worse, in any quantum experiment, they provide a significant source of decoherence, greatly increasing the difficulty of creating macroscopic quantum states. In magnetically levitated systems, this pathway of decoherence is largely removed~\cite{Romero2021}.


The extremely low damping of magnetic systems, combined with their relatively high mass and operation in low noise cryogenic environments, makes them well suited for mesoscopic probes of quantum mechanics and could provide a test to possible limits of the applicability of quantum mechanics to the macroscopic world~\cite{leggett2002,arndt2014}.
Van Waarde et al.~\cite{Waarde2016} and Vinante et al.~\cite{vinante2020} have previously realised such magnetic levitation of sub-milligram particles, in which the motional state of the particle is read out by means of superconducting quantum interference device (SQUID) detection.

%The extremely soft coupling and resulting high isolation from the environment are critical to any quantum mechanical experiment at low frequency, since even at millikelvin temperatures the bath temperature will otherwise dominate the decoherence time of any quantum state. 


%Their motion can be detected using SQUID detection of the change in flux in a nearby coil due to the particle’s motion at frequencies in the range of \SIrange{1}{100}{Hz}.
%Because the particles are levitated above a type-I superconductor, the experiments are performed at cryogenic temperatures. Together with the low damping this results in a very low force noise. These superconducting traps also provide excellent shielding from magnetic and electric forces, further shielding the probe from non-gravitational sources of noise. This, then, seems to be a promising route for combining millimeter sized test masses with detection in the hertz regime. 

In a recent publication, Westphal et al. have demonstrated gravitational coupling between two \SI{90}{mg}, \SI{1}{mm} radius, gold spheres, achieved off resonance at millihertz frequencies in a torsion balance-type geometry~\cite{aspelmeyer2021}. Recent work by Brack et al. ~\cite{brack2022} has shown the dynamical detection of gravitational coupling between two parallel beams of a  meter in size in the hertz regime. In this paper we present work with a \SI{2.4}{kg} source mass and a magnetically levitated sub-milligram test mass, giving a coupling of \SIrange{10}{30}{aN} with a force noise of $\SI{0.5}{fN/\sqrt{Hz}}$. This work provides an intermediate step towards an experiment where a small test mass senses the gravity sourced by a small source mass.

==> Results/Results.tex <==
\section{Results and  Discussion} \label{sec:results}
In figure~\ref{fig2:spectrum}B. we show the uncalibrated spectrum.
We clearly observe the six different modes corresponding to the three translational modes, and three rotational modes respectively. 
Furthermore, we see a distinct peak at 27 Hz, which we attribute to the z-mode as discussed in section~\ref{sec:setup}.
These modes were validated and calibrated by performing a magnetic drive, excited by a flux injected through the calibration transformer, as shown in figure~\ref{fig1:setup}B. 

\begin{figure}[ht]%
\centering
\includegraphics[width=\textwidth]{Results/paper_spectrum_combined.pdf}%, bb=0 0 700 500
\caption{\textbf{\emph{A}}: Force noise of the \SI{27}{Hz} mode when gravitationally driven at \SI{1.3}{mHz} detuning, overnight. \textbf{\emph{B}}: Typical resonator power spectrum. In this figure we have greyed out the regular \SI{50}{Hz} european electrical noise. Which typically has a similar power to the particle resonances.}\label{fig2:spectrum}
\end{figure}

Using this magnetic drive, we determine the decay time of the modes during the subsequent ringdown. For the \SI{26.7}{Hz} mode, we find a lower bound  $\tau = \SI{1.09e5}{s}$, or a Q factor of $Q = \SI{9.13e6}{}$. This procedure is further discussed in appendix~\ref{app:qfactortransfer}. For the other modes, we arrive at Q factors that are about an order of magnitude lower.

We test the force sensitivity of our mode by driving the \SI{26.7}{Hz} mode using the brass masses of the mass-wheel. 
The resulting excitation at one position of the wheel in the force spectrum, is shown in figure~\ref{fig2:spectrum}A. 
The calibration of this spectrum is discussed in appendix~\ref{app:qfactortransfer},~\ref{app:calibration} and~\ref{app:correction_and_conversion}. 
The resulting force noise of this z-mode is approximately $\SI{0.5}{fN/\sqrt{Hz}}$,  or equivalently, a displacement noise of $\SI{60}{pm/\sqrt{Hz}}$, in an \SI{8}{mHz} bandwidth centered around the orange dotted line that indicates the frequency of the resonance. 
Equivalently, we can determine the motion of the trap in which the particle is levitated by dividing the force noise by the spring constant of the confinement potential that keeps the particle around its equilibrium height. 
The spring constant for the z-mode was determined to be k = \SI{12e{-3}}{N/m}, resulting in a trap displacement noise of $\SI{30}{fm/\sqrt{Hz}}$.
This vibrational noise is not yet thermally limited, but rather corresponds to a mode temperature of 3 K, which we attribute to the limits of the vibration isolation inside the cryostat.

In figure~\ref{fig3:force} we show the measured gravitational interaction for different displacements of the wheel, using the method described in appendix~\ref{app:correction_and_conversion}. We also plot the phase of the masses along the wheels rotation for which the particle experiences maximal force, see figure \ref{app:phase}. For the longitudinal displacement, the vertical displacement was held at \SI{48}{} $\pm$ \SI{4}{} centimeter. In the run of vertical positions, the wheel was kept centered with respect to the trap. Included is the expected gravitational signal at the location of the magnetic particle for the z-mode of the particle, which was calculated from an analytical simulation where the mass was taken to consist of multiple point masses. From this same simulation, a systematic error bound was derived, based on an estimated systematic error, for the longitudinal run, of $\pm$5 centimeter longitudinal, $\pm$3 centimeter lateral, and $\pm$4 centimeter vertical, which were estimated from the geometry of the wheel, the mass spring system and the systems used to measure the displacements. For the vertical run, the bounds are $\pm$2 centimeter in each principal direction, based on the increased stability of the system under vertical displacement.

\begin{figure}[ht]%
\centering
\includegraphics[width=\textwidth]{Results/paper_full_combined.pdf}% , bb=0 0 850 500
\caption{\textbf{\emph{A}}: Force experienced by the mechanical resonator as a result from drive using the mass wheel, for different lateral displacement of the mass wheel relative to the particle. The dashed blue line represents the simulated gravitational force at the position of the magnetic particle as discussed in the main text. The blue area denotes the systematic uncertainty discussed in the text. A second, dashed line is plotted, which has a scaling factor of 0.35 applied, that seems to agree with the data more closely. \textbf{\emph{B}}: Similar to A, but now for a vertical displacement of the mass wheel relative to the particle, when the wheel is kept centered below the particle. Systematic bounds as discussed in the text.   \textbf{\emph{C}}: Here we see the wheel phase at which the magnetic particle experiences the strongest force, plotted against longitudinal displacement. \textbf{\emph{D}}: Similar to C, but now for a vertical displacement.\\
}\label{fig3:force}
\end{figure}

The observed signal agrees with the simulated force signal to within a factor 0.35 with a standard error of 0.02, which was determined by means of an orthogonal distance regression fit to the data.

We attribute this constant factor to the effect of the wheel on the trap. Since the centre of mass of the particle and the trap together with the holder are closely spaced, they all experience a similar gravitational gradient. For the trap, however, the frequency of the gravitational drive is far above resonance (that is: the resonance determined by the suspension of the trap and holder by springs in the form of the mass spring system), which naturally gives rise to a 180\textdegree\ phase shift in the trap's response. This phase shift means that the resulting motion of the trap leads to a suppression of the particle response.








==> Setup/Setup.tex <==
\section{Experimental setup}\label{sec:setup}
The core of the setup is a type-I superconducting trap with a magnetic particle levitated therein, as shown in Fig.~\ref{fig1:setup}b.
The trap is made of tantalum with a critical temperature of $T_c = \SI{4.48}{K}$. We perform the experiment at temperatures below \SI{100}{mK}.
The trap has an elliptical shape (\SI{4.5}{mm}$~\times$~\SI{3.5}{mm}, with the height from bottom of the trap to the coil being \SI{4.7}{mm}) to confine the modes of the levitated magnetic particle to the axial system of the trap.
The particle is composed of a set of three $\SI{0.25}{mm} \times \SI{0.25}{mm} \times \SI{0.25}{mm}$ Nd$_{2}$Fe$_{14}$B magnets that are magnetically attached North-to-South as also shown in Fig.~\ref{fig1:setup}b, and a spherical glass bead, \SI{0.25}{mm} radius, that is attached to the middle magnet using stycast. This bead is added to break the rotational symmetry of the zeppelin around the x-axis (angle $\gamma$).
Typical remnant magnetisation of Nd$_{2}$Fe$_{14}$B magnets is in the order of \SI{1.4}{T}.
The estimated mass of the full particle, as depicted in Fig.~\ref{fig1:setup}d, is \SI{0.43}{mg}.
Using the infinite plane approximation of Vinante et al. \cite{vinante2020}, we calculate an expected z-mode frequency of \SI{27}{Hz} in this geometry.

The motion of the particle results in a change of flux through a loop at the top of the trap (the pick-up loop), which is detected using a two-stage biased SQUID coupled inductively to the pick-up loop. The loop is positioned off-center so that the symmetry is broken, and all modes couple to the loop.
A third loop positioned halfway between the SQUID input loop and the pick-up loop is coupled inductively to a calibration loop. This transformer is used to calibrate the energy coupling $\beta^2$ between the detection circuit and the degrees of motion of the zeppelin, providing calibrated motion of the zeppelin from the measured flux signal.
This procedure is further described in App.~\ref{app:calibration}.

The set-up is hung by springs from a multi-stage mass spring system to shield the experiment from external vibrations, both vertical and lateral.
The bottom three masses (one aluminum, two copper) are similar in weight to the experimental setup, with a lowest resonance frequency at \SI{0.9}{Hz}.
Above that is a millikelvin mass spring system with a lowest resonance frequency of \SI{4.8}{Hz}.
We refer to Ref.~\cite{wit2019} for more details on a near identical mass-spring system and its performance in a similar dilution refrigerator.
This combination is hung from the 1K plate by a long spring. 
Thermalisation of the experiment is provided by a flattened silver wire, which is mechanically soft while providing a good thermal link.
This entire system is depicted in Fig.~\ref{fig1:setup}a. 

The cryostat as a whole is rigidly attached to a 25 metric ton concrete block, which is again placed on pneumatic dampers to limit vibrations coupling in from the building. The pulse tube cooler and the vacuum pumps for the circulation of the mixture are rigidly attached to the building through a second frame, and attached to the cryostat only by edge welded bellows and soft copper braiding to further limit external excitations from reaching the particle.

To demonstrate the force sensitivity of the system and as a proof of concept for gravitational coupling in levitated magnetic systems, we utilized an electrically driven wheel with a set of three \SI{2.45}{kg} brass masses, placed equally spaced along the outer rim.
This wheel was used to create a time dependent gravitational gradient at the resonant frequency of a selected mode of the zeppelin, in an effort to drive the motion gravitationally.
The frequency of the masses was read out optically using a laser and photodiode, in which the masses act as a mechanical shutter.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{Setup/SetupSchematic.pdf}%,bb=0 0 6000 6000]
    \caption{Schematic depiction of the experimental setup. \textbf{\emph{A}}: Multi-stage mass spring system to isolate from external vibrations, as discussed in the text. Electromagnetic shielding of the trap is discussed in appendix~\ref{app:photo}.
    \textbf{\emph{B}}: Conventions for degrees of freedom adopted from Vinante et al.~\cite{vinante2020}. Detection by SQUID as discussed in the text.  Calibration loop as discussed in the text and App.~\ref{app:calibration}. 
    \textbf{\emph{C}}: An image of: the dilution refrigerator used for the experiments, including the multi-stage mass spring system. 
    \textbf{\emph{D}}: The magnetic particle, composed of three $\SI{0.25}{mm} \times \SI{0.25}{mm} \times \SI{0.25}{mm}$ Nd$_{2}$Fe$_{14}$B magnets (SuperMagnetMan, C0005-10) magnetically attached end-to-end and a single spherical glass bead with a \SI{0.25}{mm} radius attached using Stycast to the middle of the magnets, which is used to break the symmetry of the $\gamma$ mode.
    \textbf{\emph{E}}: The trap, as placed in the aluminium holder without the shielding cylinder. The aluminium foil envelope provides additional electro-magnetic shielding between the calibration transformer and the pick-up loop.
    Further details and images of the setup are shown in Appendix~\ref{app:photo}.
    }\label{fig1:setup}
\end{figure}
